Probabilistic Offline Policy Ranking with Approximate Bayesian Computation

In practice, it is essential to compare and rank candidate policies offline before real-world deployment for safety and reliability. Prior work seeks to solve this offline policy ranking (OPR) problem through value-based methods, such as Off-policy evaluation (OPE). However, they fail to analyze special cases performance (e.g., worst or best cases), due to the lack of holistic characterization of policies performance. It is even more difficult to estimate precise policy values when the reward is not fully accessible under sparse settings. In this paper, we present Probabilistic Offline Policy Ranking (POPR), a framework to address OPR problems by leveraging expert data to characterize the probability of a candidate policy behaving like experts, and approximating its entire performance posterior distribution to help with ranking. POPR does not rely on value estimation, and the derived performance posterior can be used to distinguish candidates in worst, best, and average-cases. To estimate the posterior, we propose POPR-EABC, an Energy-based Approximate Bayesian Computation (ABC) method conducting likelihood-free inference. POPR-EABC reduces the heuristic nature of ABC by a smooth energy function, and improves the sampling efficiency by a pseudo-likelihood. We empirically demonstrate that POPR-EABC is adequate for evaluating policies in both discrete and continuous action spaces across various experiment environments, and facilitates probabilistic comparisons of candidate policies before deployment.

==> add.tex <==
\section{Multiple Expert Policies Solution \& Result}

\paragraph{Verify of Multi-expert Policy Distribution and Trajectory Variance}

We adopted 5-25 well-performed expert policies in MountainCar and Acrobot Environment, below is an example on 5 policies on MountainCar, which guarantees their variety of policies reflected by the various action preference on the same states.
% \vspace{-5mm}


\paragraph{Extension Based on Effective \oursabc}
In this part, we provide a demonstration of how to solve multiple expert policies situation as shown in Fig.~\ref{fig:extension}.
\vspace{-2mm}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.40\textwidth]{pics/mountaincar_multi_hist.png}
    \caption{Verification on the expert dataset with policy variance}
    \label{fig:variance}
\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.42\textwidth]{pics/multi_expert_figure.pdf}
    \caption{Possible Extension Based on POPR-EABC}
    \label{fig:extension}
\end{figure}

\begin{table}[thb]
\tiny
\centering
\caption{Rsults of Multiple Expert Extension on Policies Datasets
}

\begin{tabular}{ccccc}
\toprule Dataset $D_e$
& \multicolumn{2}{c}{\mcd} & \multicolumn{2}{c}{\acro} \\ 

\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                & NDCG        
                & SRCC        
                & NDCG          
                & SRCC   
\\ 
% -------- added data -------------
% \midrule
\midrule

$D_e$ (5 Experts) 
& 1.0000$_{\pm\text{0.00}}$    
& 1.0000$_{\pm\text{0.00}}$   
& 1.0000$_{\pm\text{0.00}}$   
& 1.0000$_{\pm\text{0.00}}$ \\ 

$D_e$ (10 Experts) 

& 0.9993$_{\pm\text{0.00}}$   
& 0.9809$_{\pm\text{0.03}}$ 
& 1.0000$_{\pm\text{0.00}}$    
& 1.0000$_{\pm\text{0.00}}$ \\

$D_e$ (15 Experts) 
& 0.9907 $_{\pm\text{0.01}}$    
& 0.9238$_{\pm\text{0.03}}$   
& 1.0000$_{\pm\text{0.00}}$    
& 1.0000$_{\pm\text{0.00}}$ \\

$D_e$ (20 Experts) 
& 0.9971 $_{\pm\text{0.01}}$    
& 0.9428$_{\pm\text{0.09}}$   
& 1.0000$_{\pm\text{0.00}}$    
& 1.0000$_{\pm\text{0.00}}$ \\

$D_e$ (25 Experts) 
& 0.9981 $_{\pm\text{0.01}}$    
& 0.9429$_{\pm\text{0.00}}$   
& 0.9999$_{\pm\text{0.00}}$    
& 0.9762$_{\pm\text{0.00}}$ \\
% \midrule
% $std$ (25 Experts) 
% & 0.9981 $_{\pm\text{0.01}}$    
% & 0.9429$_{\pm\text{0.00}}$   
% & 0.9999$_{\pm\text{0.00}}$    
% & 0.9762$_{\pm\text{0.00}}$ \\

\bottomrule
\end{tabular}
\end{table}

\section{Extra Experiment Report}



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.50\textwidth]{pics/posterior.png}
    \caption{Posterior Comparison Between Candidate Policies Shows POPR-EABC is Effective in Estimating Performance and Helpful for Ranking}
    \label{fig:enter-label}
\end{figure}



\begin{table}[h!]
\centering
\caption{Rsults of BipdedalWalker}
\begin{tabular}{ccc}
\toprule Baselines
& \multicolumn{2}{c}{\bip} \\ 

\cmidrule(lr){2-3}
                & NDCG        
                & SRCC     \\ 
\midrule

% -------- added data -------------
% \midrule

\fqe  
& 0.7196$_{\pm\text{0.02}}$    
& 0.3452$_{\pm\text{0.26}}$  \\ 

\tree

& 0.6869$_{\pm\text{0.12}}$   
& 0.3177$_{\pm\text{0.25}}$  \\

\Qpi
& 0.7023$_{\pm\text{0.08}}$    
& 0.1975$_{\pm\text{0.22}}$  \\

\MBased
& 0.6128$_{\pm\text{0.11}}$    
& -0.2006$_{\pm\text{0.41}}$  \\

\dice
& 0.8192$_{\pm\text{0.04}}$    
& 0.1437$_{\pm\text{0.18}}$  \\

\midrule
\agr
& 0.8022$_{\pm\text{0.13}}$    
& 0.5417$_{\pm\text{0.15}}$  \\

\midrule
\oursabc
& 0.8990$_{\pm\text{0.05}}$    
& 0.5816$_{\pm\text{0.03}}$  \\

\bottomrule
\end{tabular}
\end{table}

% \vfill


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.49\textwidth]{pics/extra1.pdf}
    \vspace{-3mm}
    \caption{Extra experiments on SOPR policies datasets}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.3\textwidth]{pics/HalfCheetah_set1.png}
    \vspace{-3mm}
    \caption{Extra experiments on SOPR policies datasets}
    \label{fig:enter-label}
\end{figure}



\paragraph{Baseline Comparison to SOPR}




\paragraph{BipedalWalker environment}
Below we report extra results of baseline methods on the BipedalWalker environment. 

